No Privacy in the Electronics Repair Industry

Electronics repair and service providers offer a range of services to computing device owners across North America -- from software installation to hardware repair. Device owners obtain these services and leave their device along with their access credentials at the mercy of technicians, which leads to privacy concerns for owners' personal data. We conduct a comprehensive four-part study to measure the state of privacy in the electronics repair industry. First, through a field study with 18 service providers, we uncover that most service providers do not have any privacy policy or controls to safeguard device owners' personal data from snooping by technicians. Second, we drop rigged devices for repair at 16 service providers and collect data on widespread privacy violations by technicians, including snooping on personal data, copying data off the device, and removing tracks of snooping activities. Third, we conduct an online survey (n=112) to collect data on customers' experiences when getting devices repaired. Fourth, we invite a subset of survey respondents (n=30) for semi-structured interviews to establish a deeper understanding of their experiences and identify potential solutions to curtail privacy violations by technicians. We apply our findings to discuss possible controls and actions different stakeholders and regulatory agencies should take to improve the state of privacy in the repair industry.

==> Study2.tex <==
\section{Study 1: Repair Privacy Policies and Procedures}
\label{study1}

\subsection{Methodology}
In stage one, we visited repair shops and attempted to get a battery replaced on either a phone or laptop. This type of repair was chosen as it should not require the technician gain access to the users personal data. Therefore, no pin or password should be required by the shops. Additionally, a device with a bad battery can still appear normal so any device that was brought in could have this problem. To ensure that the technicians didn't need access to the software of the computer we ensured the places that we only wanted the battery replaced. Not a diagnostic scan to see if the device needed a new battery. While going through the process of the repair questions surrounding security policies and procedures were asked. Specifically, around if there was a security policy and why a pin/password is required if it was requested by the technician. Additionally, we looked for any policies or procedures that the shops had posted. Within 10 minutes of leaving the store we would fill out a survey that asked about the shops procedure and would note down anything else of concern. We would then re-enter the store and try to cancel the repair. This was done in order to save money as we didn't need the actual device to be fixed. The shops that were selected were separated into 3 categories (big box, chains, mom n' pop). A mom n' pop store was defined by any store that had one physical location. These shops also had to have a google rating of 3.5 or more stars. A chain was defined as any store that had 2 or more physical locations which were located in different cities. A big box store was defined as any publicly traded company with shops across North America. 

%Add "Quotations are from repair centre representatives unless otherwise noted." Add about manufacture repairs being initiated online (requirement)
    
\begin{table}[t]
\caption{Repair Centres}
\label{tab:1-RepairCenters}
\centering
\small\addtolength{\tabcolsep}{-3.75pt} \renewcommand{\arraystretch}{1.05}
\begin{tabular}{cccc}

\multicolumn{4}{c}{{\bf n = 16}} \\ \hline

\multicolumn{4}{c}{{\bf Centre Type}} \\
\emph{Local} & \emph{Regional} & \emph{National} & \emph{Manufacturer} \\
4 & 6 & 3 & 3 \\ \hline

\multicolumn{4}{c}{{\bf Device Type}} \\
&\emph{Laptop} & \emph{Smartphone}&      \\
&13 & 3& \\ \hline 

\end{tabular}

\end{table}

    
\subsection{Results}

\subsubsection{Privacy Policies}

